Robust Bang-Off-Bang Low-Thrust Guidance Using Model Predictive Static Programming

Model Predictive Static Programming (MPSP) was always used under the assumption of continuous control, which impedes it for applications with bang-off-bang control directly. In this paper, MPSP is employed for the first time as a guidance scheme for low-thrust transfers with bang-off-bang control where the fuel-optimal trajectory is used as the nominal solution. In our method, dynamical equations in Cartesian coordinates are augmented by the mass costate equation, while the unconstrained velocity costate vector is used as control variable, and is expressed as a combination of Fourier basis functions with corresponding weights. A two-loop MPSP algorithm is designed where the weights and the initial mass costate are updated in the inner loop and continuation is conducted on the outer loop in case of large perturbations. The sensitivity matrix (SM) is recursively calculated using analytical derivatives and SM at switching points is compensated based on calculus of variations. An sample interplanetary CubeSat mission to an asteroid is used as study case to illustrate the effectiveness of the method developed.

==> ToC.tex <==
Considering that the guidance algorithm maybe required to implement during the flight, the thrust angle should continuously vary from current status of the thrust angle. This poses the continuation constraints on the control variable. In this work, the state-of-the-art Theory of Connections (ToC) is applied to generate the control representation~\cite{mortari2017theory}. ToC mainly investigates the arbitrary connections between points, through constructing a constrained function expressed in terms of an auxiliary function~\cite{mortari2017theory}. It has the property that no matter what the auxiliary function is selected, the constrained function always satisfies prescribed set of constraints. Take a scalar constrained function as an example
\begin{equation}
\label{eqs:ToC_eg}
f(\eta) = g(\eta) + (f_0 - g_0) + (\eta - \eta_0)(f^\prime_0 - g^\prime_0)
\end{equation}
where $f(\eta)$ and $g(\eta)$ are called constrained function and auxiliary function respectively, $\eta \in \left[\eta_0, \eta_f \right]$ is the independent variable and $(\cdot)^\prime$ is the derivative w.r.t $\eta$. It is easy to verify that Eq.\ \eqref{eqs:ToC_eg} has the property that no matter what $g(\eta)$, it always satisfies $f(\eta_0) = f_0$ and $f^\prime(\eta_0) = f^\prime_0$. The constrained function is the generalization of interpolation formulae, on that it is not the interpolating expression for a class of functions (e.g., Lagrange polynomials used in Lagrange interpolation) but for all functions~\cite{mortari2017theory}. Through expressing control profile as a constrained function, the control constraint can be automatically ensured.


The extension from the scalar constrained function to the multi-dimensional constrained function is used for the expression of the control profile. The auxiliary function is expressed by basis functions. The control is expressed as
\begin{equation}
\label{eq:CF_1}
\vect U_k^i(\eta) = \vect P_k^i(\eta) \vect\epsilon + \vect Q_k^i(\eta)
\end{equation}
where $\epsilon$ is the weight to the basis functions. The detail expressions of $\vect P(\eta)$ and $\vect Q(\eta)$ are based on the initial constraints. Three cases are considered as follows.
\begin{enumerate}
	\item Without initial constraints
	\begin{equation}
	\vect P(\eta) = 
	\begin{bmatrix}
	\vect h^\top(\eta) & & &\\
	& \vect h^\top(\eta) & &\\
	& & & \vect h^\top(\eta)
	\end{bmatrix}, \quad
	\vect Q(\eta) = \vect 0_{3 \times 1}
	\end{equation}
	where $\vect h(\eta)$ is the collection of different orders of basis functions.
	\item With initial constraint $\vect U(\eta_0) = \vect U_0$
	\begin{equation}
	\vect P(\eta) = 
	\begin{bmatrix}
	(\vect h(\eta) - \vect h_0)^\top & & &\\
	& (\vect h(\eta) - \vect h_0)^\top & &\\
	& & & (\vect h(\eta) - \vect h_0)^\top
	\end{bmatrix}, \quad
	\vect Q(\eta) = \vect U_0
	\end{equation}
	\item With initial constraints $\vect U(\eta_0) = \vect U_0$ and $\vect U^\prime(\eta_0) = \vect U_0^\prime$
	\begin{equation}
	\begin{aligned}
	\vect P(\eta)& = 
	\begin{bmatrix}
	(\vect h(\eta) - \vect h_0 - (\eta - \eta_0)\vect h^\prime_0)^\top & & &\\
	& (\vect h(\eta) - \vect h_0 - (\eta - \eta_0)\vect h^\prime_0)^\top & &\\
	& & & (\vect h(\eta) - \vect h_0 - (\eta - \eta_0)\vect h^\prime_0)^\top
	\end{bmatrix}, \\ \quad
	\vect Q(\eta)& = \vect U_0 + (\eta - \eta_0)\vect U_0^\prime
	\end{aligned}
	\end{equation} 
\end{enumerate}

The $\eta$ range is determined by the basis functions chosen. The linear projection of $\eta$ w.r.t time $t$ is used as
\begin{equation}
\eta = \dfrac{\eta_f-\eta_0}{t_f-t_0}\left(t-t_0\right) + \eta_0
\end{equation}



